Towards Fundamental Limits of Multi-armed Bandits with Random Walk Feedback

In this paper, we consider a new Multi-Armed Bandit (MAB) problem where arms are nodes in an unknown and possibly changing graph, and the agent (i) initiates random walks over the graph by pulling arms, (ii) observes the random walk trajectories, and (iii) receives rewards equal to the lengths of the walks. We provide a comprehensive understanding of this problem by studying both the stochastic and the adversarial setting. We show that this problem is not easier than a standard MAB in an information theoretical sense, although additional information is available through random walk trajectories. Behaviors of bandit algorithms on this problem are also studied.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> tex/abstract.tex <==
In this paper, we consider a new Multi-Armed Bandit (MAB) problem where arms are nodes in an unknown and possibly changing graph, and the agent (i) initiates random walks over the graph by pulling arms, (ii) observes the random walk trajectories, and (iii) receives rewards equal to the lengths of the walks. We provide a comprehensive understanding of this problem by studying both the stochastic and the adversarial setting. In the stochastic setting, we show that this problem is not easier than a standard MAB, although additional information is available through random walk trajectories. In the adversarial setting, we show that an extension of the exponential weight algorithm can achieve a regret bound of order $\widetilde{\mathcal{O}} \left( \sqrt{ \kappa T}\right) $, where $\kappa$ is a constant that depends on the structure of the graph, instead of the number of arms.

==> tex/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Some are in the Appendix due to space limit.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{They are included as supplementary materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? 
    \answerYes{Please see the supplementary materials. } 
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We only run light experiments.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{We do not use existing dataset.}
  \item Did you mention the license of the assets?
    \answerNA{We do not use existing dataset.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{We are studying online learning problems. The simulation and environment is available in the code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We do not use existing dataset.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We do not use existing dataset.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tex/figure-lower.tex <==
\begin{figure}[ht!]
    \centering
    % \includegraphics{}
    % \caption{Caption}
%    \subfloat[]{
    \begin{tikzpicture}[transform shape]
  \node[draw, circle,inner sep=0.2cm] at (0, 0)   (a) {1};
  \node[draw, circle,inner sep=0.2cm] at (3, 0)   (b) {2};
%  \node[draw, circle,inner sep=0.2cm] at (1.5, 1.732 * 1.5)   (c) {3};
  \node[draw, circle,inner sep=0.2cm, fill=black] at (1.5, 1.732 * 1.5)   (tar) {}; 
  
  \path (b) edge (a) {};
%  \path (b) edge (c) {};
%  \path (c) edge (a) {};
  
  \path (a) edge (tar) {};
  \path (b) edge (tar) {};
%  \path (c) edge (tar) {};
  
  \draw (a) to [out=240,in=180,looseness=8] (a) {};
  \draw (b) to [out=-60,in=0,looseness=8] (b) {};
%  \draw (c) to [out=90-30,in=90+30,looseness=8] (c) {};
\end{tikzpicture}
%}
%\subfloat[]{ \begin{tikzpicture}[transform shape]
%  %the multiplication with floats is not possible. Thus I split the loop in two.
%%   \node[draw,circle,inner sep=0.25cm] at (0,0)
%  \node[draw, circle,inner sep=0.2cm] at (0, 0)   (a) {1};
%  \node[draw, circle,inner sep=0.2cm] at (3, 0)   (b) {2};
%  \node[draw, circle,inner sep=0.2cm] at (1.5, 1.732 * 1.5)   (c) {3};
%  \node[draw, circle,inner sep=0.2cm, fill=black] at (1.5, 1.732/2)   (tar) {}; 
%  
%%   \path (b) edge (a) {};
%%   \path (b) edge (c) {};
%%   \path (c) edge (a) {};
%  
%  \path (a) edge (tar) {};
%  \path (b) edge (tar) {};
%  \path (c) edge (tar) {};
%  
%  \draw (a) to [out=240,in=180,looseness=8] (a) {};
%  \draw (b) to [out=-60,in=0,looseness=8] (b) {};
%  \draw (c) to [out=90-30,in=90+30,looseness=8] (c) {};
%
%\end{tikzpicture}}
    
    \caption{\label{fig:lower-bound}}
\end{figure}

==> tex/rebuttal.tex <==
Dear Reviewers, Thanks for your valuable feedback. Please find below our response to your kind feedback. 

\noindent To \textbf{R1:} We're honored that you enjoyed reading our paper. Thanks for the advice that we should cite more literature on random walks, the pointers to typos and advice on writing and graphing. We will revise the paper accordingly. 

\noindent To \textbf{R2:} Thanks for the feedback. As for the motivation, one can use our method for online influence maximization problem \cite{kempe2003maximizing} in computational social networks. The influence maximization model captures many important applications. For example, recommending a movie to a person of high influence (in a social network) might result in more people in her circle watching that movie. As another example, a scientific question raised by highly cited authors (in a citation network) may grasp more attention than questions (of the same quality) raised by less cited authors. Thanks for pointing out that more experiments are helpful. Please see some additional experiments in the figure at the end of this file. 

As for whether the $\Omega (\sqrt{T})$ lower bound contradicts the $ O (\log T) $ upper bound, the answer is no. Upper bounds of order $O(\log T)$ is referred to as instance-dependent upper bounds. Such $O(\log T)$ bounds depend on the intrinsics of the specific problem instance. Contrastingly, upper bounds of order $O(\sqrt{ T })$ are referred to as instance-independent upper bound. Such $O(\sqrt{ T })$ bounds hold true for all problem instances (with the same number of arms). Lower bounds that match the $O(\log {T})$ (resp. $O(\sqrt{T})$) bound is usually referred to as asymptotic (resp. worst-case/mini-max/information-theoretical) lower bounds. These bounds for standard MAB are established results. We show that our problem setting can be as hard as standard MAB in the worst case sense, even though much more information is available. 



% The lower bound result looks non-trivial. But, at the same time, by reducing the problem to the stochastic MAB, O(log T) bound is possible by e.g., UCB. Could you explain what the intuition for requiring Omega(\sqrt T) regret? For example, magnitude of reward is O(\sqrt{T}) or something?



% A relatively recent paper on influence maximization is \citep{}. 
% that we should cite more literature on random walks, the pointers to typos and advice on writing and graphing. We will revise the paper accordingly. 


\noindent To \textbf{R3:} Thanks for the feedback. Please see our response to R2 for discussions on the motivation. This problem setting is proposed by us. Thanks for pointing out that more experiments can be helpful. Please find some additional empirical study in the figure at the end of this file. 


\noindent To \textbf{R4:} Thanks for the feedback. Firstly, we do not agree that an $\Omega (\sqrt{T})$ lower bound for the stochastic case is intuitive. Quite the opposite is true. If one can observe reward samples from all arms no matter what arms she plays, then the estimates of all arms concentrate quickly, regardless of what policy is executed. In this case, one can play arms arbitrarily until concentrations around all arms are tight, and then greedily play the best arm. This would give a constant regret bound. In our stochastic setting, where the environment can carry much more information than just reward samples of all arms (via random walks), one would expect a lower bound smaller than $\Omega(\sqrt{T})$. We prove that this intuition is wrong, and an $\Omega(\sqrt{T})$ can be established in the information theoretical sense. For the stochastic case, perhaps an $O (\sqrt{T})$ \textit{upper bound} is somewhat straight-forward, but an $\Omega (\sqrt{T})$ \textit{lower bound} is not. 

% To the best of our knowledge, our adversarial setting is not covered by any previous work. \textcolor{red}{what's the point here}
% cannot be reduced to any existing setting. 
% One might argue that our adversarial setting is re
% Perhaps the closest previous work is the  \textcolor{red}{maybe more words here}. 

The bounds are all tight in terms of $T$ (up to logarithmic factors). The instance-independent $O (\sqrt{T})$ upper bound for the stochastic setting is tight, since we prove an $\Omega (\sqrt{T})$ lower bound in Theorem 1. The instance-independent upper bound is constant, which means it must be tight in terms of $T$. We appreciate you raising the question regarding the instance-dependent upper bounds for the stochastic setting, since they only appear in the supplementary materials. 
The bounds for the adversarial setting are also tight (up to logarithmic factors) in terms of $T$. They are both transition-dependent (or graph-dependent in your terminology) as well. Perhaps it is the missing of explanation of $p$ in the theorem statement that caused the confusion. The sentence ``... a transition probability matrix, such that ... '' should be corrected to ``... a transition probability matrix whose entries are all $p$ ($Kp < 1$), such that ... ''. This lower bound is transition-dependent, at least when the transition graph is symmetric. We will correct this typo and add discussions on this. 
% Since the adversary can only alter the edge length, the lower bound must be derived with the transition probability fixed. 
% Sorry for the confusion 
% . We will add more discussions on this. 

We want to emphasize that, for the adversarial setting, both the upper bound and the lower bound are high probability bounds, which requires much more care and effort than standard expectation bounds. We think these high probability bounds are solid contributions since the problem setting is new. 

As for whether the algorithm implementation needs prior knowledge on $\kappa$, the answer is no. In practice, it is sufficient to choose the parameters $\eta$ and $\beta$ to be reasonably small. The knowledge of the $\eta$ and $\beta$ is for the analysis only. Thanks for pointing out that the appearance of $\kappa$ in the algorithm pseudo-code could cause confusion. We will make revisions to clarify this. 



% We really appreciate the effort of examining
% While it is true that an instance-dependent type lower bound would be very interesting, we think our current analysis . 
% Perhaps the closest previous adversarial semi-bandit works are those with graph feedback. 
% The 
% the player knows whether playing arm $ i $ reveals information about arm $j$. For example, the works. In our setting, this quantity needs to be estimated. 
% unlike existing adversarial semi-bandit problems where feedback structure, our algorithm does not require any  
% our setting requires estimating feedback the structure probability the while controlling the adversarial regret, whereas existing works assume that the feedback structure is known. 

% For the third concern, we . 

% -----------------

\begin{figure}[h!]
    \centering
    \includegraphics[scale = 0.57]{figures/additional_exp.png}
    \caption{This figure shows the comparison between Algorithm 1 and the EXP3 algorithm. Each line plot summarizes 10 runs. The solid line is the mean regret and the shaded area around each line indicates one standard deviation above and below the mean regret. This figure shows that our method outperforms the EXP3 algorithm. \label{fig:add}} 
\end{figure} 

==> tex/ucb.tex <==


% \begin{theorem} 
%     \label{thm:no-gap} 
%     Let $T$ be any positive integer. Under Assumption \ref{assumption:transition}, Algorithm \ref{alg:opt} admits a regret of order 
% 	\begin{align*}
% 	    \Reg (T) = \widetilde{\mathcal{O}} \( \min \left\{ \frac{1}{ (1 - \rho)^2} \sqrt{ \frac{T}{\alpha}} \, , \; \frac{1}{ (1 - \rho)^2} \sqrt{ K  T } \right\} \) ,
% 	\end{align*}
% 	where $\alpha = \min_{v \in V} \alpha_v$ ($\alpha_v$ defined in Definition \ref{def:centrality}). 
% \end{theorem} 

% \begin{theorem} 
% \label{thm:opt} 
% On a problem instance that satisfies Assumption \ref{assumption:transition}, Algorithm \ref{alg:opt} achieves constant regret of order $\widetilde{\mathcal{O}} \( \sum_{v: \Delta_v > 0} \( \Delta_v + \frac{1}{  (1 - \rho)^2 \Delta_v }  \) \) $, where $\widetilde{\mathcal{O}} $ omits absolute constants and logarithmic dependence on problem intrinsics. 
% \end{theorem} 

% More details on Theorems \ref{thm:no-gap} and \ref{thm:opt} are in Appendices \ref{app:no-gap} and \ref{app:gap} for completeness. 


% \subsection{Concentrations of Estimators}
% \label{app:concen}

% \textbf{\textit{Note.}} In the stochastic setting, the graph is time-invariant. For easier reference, we define random variables $Z_v$ such that $ Z_v $ has the same distribution as $ \L \( \P_{t,v} \) $ for all $t$. Then, in the stochastic setting, 
% \begin{align}
%     \Delta_v = \E \[ Z_{v^*}  \] -  \E \[  Z_{v} \], \quad \text{ where } \quad v^* \in \arg\max_{v} \E \[ Z_{v} \]. 
% \end{align}


% In this part, we derive concentration bounds for hitting time estimators $\wt{Z}_{v,n}$. 
% % To prove Theorem \ref{thm:greedy}, we first show that the random variables $Y_{ v, k_{v,i}  }$ are sub-exponential for any $(v,i)$. 
% To start with, we show that the hitting times are sub-exponential. 
% % Since the problem is stochastic, we use $Z_i$ to denote $Z_{t,i}$ for all $t \in \mathbb{N}$ and $i \in [K]$. 

% \begin{lemma} \label{lem:sub-exp}
%      For any $v \in [K]$, $i = 1,2,\cdots$ and any integer $ x > 0 $, we have 
%     \begin{align}
% 		\Pr \( Y_{v,k_{v,i}} \ge x \) 
% 		\le  \frac{ \rho^{x} }{1 - \rho}. \nonumber
% 	\end{align} 
% 	where $\rho$ is defined in Assumption \ref{assumption:transition}. 
% \end{lemma}

% \begin{proof}
%     Let $M$ be the transition matrix among transient nodes. 
%     Since for any $(v, i, x)$,  
%     \begin{align*}
%         &\left\{  Y_{v,k_{v,i}} \ge x \right\} \\
%         =& \left\{ \text{a random walk starting from $v$ does not reach the absorbing node in $x$ steps} \right\}, 
%     \end{align*} 
%     we have,
%     \begin{align}
%         \Pr \( Y_{v,k_{v,i}} \ge x \) 
%         &\le \Pr \( \{ \text{random walk starting from $v$ does not terminate in $x$ steps} \} \) \nonumber \\
%         &= \sum_{h=x}^\infty \Pr \( \{ \text{random walk starting from $v$ terminates at step $h$} \} \) .  \label{eq:1}
%     \end{align} 
%     Writing out the probability in (\ref{eq:1}) gives 
%     \begin{align*}
%         \Pr \( Y_{v,k_{v,i}} \ge x \) 
%         &\le \sum_{l=x}^\infty \sum_{ j = 1 }^K \[ M^l \]_{ij} 
%         \le \sum_{l=x}^\infty \| M^l \|_\infty 
%         \le \sum_{l=x}^\infty \rho^l 
%         \le \frac{ \rho^x }{1 - \rho}. 
%     \end{align*}
% \end{proof}

% For the concentration results, we use Lemmas \ref{lem:extended-azuma} and \ref{lem:concentration-no-truncation}. 

% \begin{lemma}[Proposition 34 by \cite{tao2015random}] \label{lem:extended-azuma}
% 	Consider a martingale sequence $ X_1, X_2,  \cdots$ adapted to filtration $\mathcal{F}_1, \mathcal{F}_2 \cdots$. For constants $c_1, c_2, \cdots < \infty$, we have 
% 	\begin{align}
% 		&\mathbb{P} \left(  \left\rvert X_n - X_0 \right\rvert > \lambda \sqrt{ \sum_{i=1}^n c_i^2 } \right) \le 2 \exp \left( - \frac{\lambda^2}{ 2  } \right) + \sum_{i=1}^n \mathbb{P} \left( \left\rvert X_i - X_{i-1} \right\rvert > c_i \right). 
% 	\end{align} 
% \end{lemma} 


% Lemma \ref{lem:extended-azuma} is an extension of the Azuma's inequality with an extra term bounding the probability of any term in the martingale difference sequence being unbounded. 

% \begin{lemma}   
%     \label{lem:concentration-no-truncation}
% % 	Let $Z_v$ be the hitting time random variable from $ v $ to $*$. 
% 	For any transient node $v \in [K]$, if $N_t^+(v)>0$, we have 
% 	\begin{align} 
% 		\Pr \( \left\rvert \wt{Z}_{v, {N}_t^+ (v) } - \E \[ \L \( \P_{s,v} \) \] \right\rvert \ge \sqrt{ \frac{  8 \xi_t \log t }{  {N}_t^+ (v) } }  \) \le 3 t^{-4}, \quad \forall s,t \in \mathbb{N}_+ \label{eq:sub-exp-con-t}
% 	\end{align} 
% 	where $ \xi_t = \xit$. 
	
% \end{lemma} 

% \begin{proof}
%     By Lemma \ref{lem:sub-exp}, 
%     we have,  when $x \ge \E \[ Y_{ v, k_{v,i}  } \]$,
%     \begin{align}
%         \Pr \( \big\rvert Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \big\rvert \ge x \) 
%         \le& \Pr \( Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \ge x \) + \Pr \( - Y_{ v, k_{v,i}  } + \E \[ Y_{ v, k_{v,i}  } \] \ge x \) \nonumber \\
%         \le& \Pr \(  Y_{ v, k_{v,i}  }  \ge x \) + \Pr \(  Y_{ v, k_{v,i}  }  \le \E \[ Y_{ v, k_{v,i}  } \] - x \) \tag{the second term is zero.} \\ 
%         \le& \frac{ \rho^x }{ 1 - \rho } 
%         \label{eq:sub-exp}. 
%     \end{align}
    
%     Also by Lemma \ref{lem:sub-exp}, $\E \[ Y_{ v, k_{v,i}  } \] = \sum_{x=0}^\infty \Pr \( Y_{v,k_{v,i}} \ge x \) \le 1 + \sum_{x=1}^\infty \frac{\rho^x}{1 - \rho} \le 1 + \frac{\rho}{ (1 - \rho)^2 } $. 
%     Since (\ref{eq:sub-exp}) is true only for $ x \ge \E \[ Y_{ v, k_{v,i}  } \] $, by setting 
%     \begin{align*}
%         \xi_t = \xit, 
%     \end{align*}
%     we have 
%     \begin{align}
%         \Pr \( \left\rvert Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \right\rvert \ge \xi_t \) 
%         \le t^{-5}.  \label{eq:sub-exp-2} 
%     \end{align}
    
%     Applying Lemma \ref{lem:extended-azuma} gives
%     \begin{align}
%         &\Pr \( \left\rvert \sum_{i=1}^{ {N}_t^+ (v) } \big[ Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \big] \right\rvert \ge \lambda \sqrt{ \sum_{i=1}^{{N}_t^+ (v) } \xi_t } \) \nonumber \\
%         \le& 2 \exp \( \frac{ - \lambda^2 }{ 2 } \) + \sum_{i=1}^{{N}_t^+ (v)} \Pr \( \left\rvert Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \right\rvert \ge \xi_t \) \nonumber \\
%         \le& 2 \exp \( \frac{ - \lambda^2}{ 2 } \) + t^{-4} . \label{eq:sub-exp-lambda}
%     \end{align}  
    
%     At time $t$, we set $ \lambda = \sqrt{ 8 \log t } $, and from (\ref{eq:sub-exp-lambda}) we get 
%     \begin{align*}
%         &\Pr \( \left\rvert \wt{Z}_{v, {N}_t^+ (v) } - \E \[ \wt{Z}_{v, {N}_t^+ (v) } \] \right\rvert \ge  \sqrt{ \frac{ 8 \xi_t \log t  }{ {N}_t^+ (v) } }  \)  \\
%         &= \Pr \( \left\rvert  \sum_{i=1}^{ {N}_t^+ (v) } \big[ Y_{ v, k_{v,i}  } - \E \[ Y_{ v, k_{v,i}  } \] \big] \right\rvert \ge \sqrt{ 8 \log t }  \sqrt{ \sum_{i=1}^{{N}_t^+ (v) } \xi_t  } \) \le 3 t^{-4}. 
%     \end{align*} 
%     We now conclude the proof by using $ \E \[ \wt{Z}_{v, {N}_t^+ (v) }\] = \E \[ \L \( \P_{s,v} \) \] $ for all $s,t \in \mathbb{N_+} $. 
% \end{proof} 


% \subsection{Proof of Theorem \ref{thm:no-gap}}
% \label{app:no-gap}
% Firstly, we bound the step regret at time $t$ by the confidence radius at time $t$, as is common in bandit regret analysis (e.g., \cite{srinivas2010gaussian}). 

% \begin{lemma} \label{lem:single-regret}
% 	With probability at least $1 - \frac{2}{t^4}$, Algorithm \ref{alg:opt} satisfies, for any $t \in \mathbb{N}$, 
% 	\begin{align}
% 	    \E \[ Z_{v^*} \] - \E \[ Z_{J_t} \] \le \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho)^2 \sqrt{ N_t^+ (J_t) } } \) ,
% 	   % , \quad  \text{where} \quad \wh{C}_{ {N}_t^+ (v), t }:= \CT{ {N}_t^+ (v) }
% 	\end{align} 
% 	where $ \mathcal{O} $ omits absolute constants and logarithmic factors in problem intrinsics. 
% \end{lemma}
 
% \begin{proof} 
%     By Lemma \ref{lem:concentration-no-truncation}, with probability at least $1 - \frac{2}{t^4}$, we have 
% 	\begin{align}
% 		\E \[ Z_{J_t} \] \le \wt{Z}_{ J_t, {N}_t^+  (J_t)  } + \wt{C}_{ {N}_t^+ (J_t) , t } \quad \text{and} \quad \E \[ Z_{v^*} \] \ge \wt{Z}_{ v^*, {N}_t^+  (v^*)  } - \wt{C}_{ {N}_t^+ (v^*) , t } 
% 	\end{align} 
% 	Thus, with probability at least $1 - \frac{2}{t^4}$, 
% 	\begin{align}
% 		\E \[ Z_{J_t} \] - \E \[ Z_{v^*} \] &= \wt{Z}_{ J_t, {N}_t^+  (J_t)  } + \wt{C}_{ {N}_t^+ (J_t), t }
% 		- \( \wt{Z}_{ v^*, {N}_t^+  (v^*)  } + \wt{C}_{ {N}_t^+ (v^*) , t } \) \\
% 		&\le \wt{Z}_{ J_t, {N}_t^+  (J_t)  } + \wt{C}_{{N}_t^+ (J_t), t} - \( \wt{Z}_{ J_t, {N}_t^+  (J_t) } + \wt{C}_{ {N}_t^+ (J_t) , t } \) \label{eq:use-greedy} \\
% 		&\le 2 \wt{C}_{ {N}_t^+ (J_t) , t} \\
% 		&\le \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho )^2 \sqrt{ N_t^+ (J_t) } } \)  , 
% 	\end{align}  
% 	where (\ref{eq:use-greedy}) uses that $J_t \in \arg\max_{v \in V} \[ \wt{Z}_{ J_t, {N}_t^+ (v) } + \wt{C}_{ {N}_t^+ (v), t } \]$. 
% \end{proof} 

% \begin{theoremn} [\ref{thm:no-gap}]
%     Let $T$ be any positive integer. Under Assumption \ref{assumption:transition}, Algorithm \ref{alg:opt} admits regret of order 
% 	\begin{align*}
% 	Reg (T) = \widetilde{\mathcal{O}} \( \min \left\{ \frac{1}{ (1 - \rho)^2} \sqrt{ \frac{T}{\alpha}} \, , \; \frac{1}{ (1 - \rho)^2} \sqrt{ m  T } \right\} \) , \end{align*}
% 	where $\alpha = \min_{v \in V} \alpha_v$, and $\alpha_v$ is defined in Definition \ref{def:centrality}, and $\wt{ \mathcal{O} }$ omits poly-logarithmical factors in $T$. 
% \end{theoremn} 

% % We shall note that the problem intrinsics that show up 
% In this bound the dependence on optimality gaps $\Delta_v$ are removed and all problem intrinsics are global. In other words, Algorithm \ref{alg:opt} achieves this regret rate no matter how identical the nodes are. 
	
% \begin{proof} 
    
%     \textbf{Part I: $\Reg (T) = \widetilde{\mathcal{O}} \(   \frac{ 1 }{ (1 - \rho)^2 } \sqrt{ \frac{ T }{\alpha} } \) $. } 
% 	For any $t, T \in \mathbb{N}$, consider events
%     \begin{align} 
% 		\wt{\mathcal{E}}_t &:= \bigg\{ \E \[ Z_{J_t} \] \le \wt{Z}_{ J_t, {N}_t^+(J_t) } + \wt{C}_{ {N}_t^+ (J_t), t} \quad \text{and} \quad \E \[ Z_{v^*} \] \ge \wt{Z}_{ v^*, {N}_t^+(v^*) } - \wt{C}_{ {N}_t^+ (v^*) , t } \bigg\}, \nonumber \\ 
% 		\mathcal{E} &:= \left\{ {N}_t^+ (v) - N_t(v) - (t - N_t(v))  \alpha_{v} \ge - \sqrt{ t \log \left( m T \right) } \quad \forall t \in [T], v \in V \right\}. \nonumber
% 	\end{align} 
% 	By Lemmas \ref{lem:concentration-no-truncation} and \ref{lem:event}, 
% 	\begin{align}
% 	    \Pr \( \wt{\mathcal{E}}_t \cap \mathcal{E} \) \ge 1 - \frac{4}{t^4} - \frac{1}{T}. \label{eq:prob}
% 	\end{align}
%     By Lemma \ref{lem:sub-exp}, 
%     \begin{align} 
% 	    \E \[ Z_{v^*} \] = \sum_{ x= 0 }^\infty \Pr \( Z_{v^*} > x \) \le 1 + \frac{ \rho }{ \( 1 - \rho \)^2 }.  \label{eq:mean-bound} 
% 	\end{align} 
% 	Thus, by (\ref{eq:prob}), (\ref{eq:mean-bound}), we have 
% 	\begin{align} 
% 		\Reg (T) &= \sum_{ t=1 }^T \( \E \[ Z_{v^*} \] - \E \[ Z_{J_t} \] \) \nonumber \\ 
% 		&\le \left\lceil \frac{\log T}{ \min_v \alpha_v^2 } \right\rceil \cdot \E \[ Z_{v^*} \] + \sum_{ t=\left\lceil \frac{\log T}{ \min_v \alpha_v^2 } \right\rceil }^T \E \[ Z_{v^*} - Z_{J_t} \bigg\rvert \wt{\mathcal{E}}_t \cap \mathcal{E} \] \Pr \( \wt{\mathcal{E}}_t \cap \mathcal{E}  \) \nonumber \\ 
% 		&\qquad + \E \[ \sum_{ t=1 }^T  \( Z_{v^*} - Z_{J_t} \) \bigg\rvert \overline{ \wt{\mathcal{E}}_t \cap \mathcal{E} } \] \( 1 - \Pr \( \wt{\mathcal{E}}_t \cap \mathcal{E} \) \) \nonumber \\ 
% 		&\le \left\lceil \frac{\log T}{ \min_v \alpha_v^2 } \right\rceil \cdot \frac{ \rho }{ \( 1 - \rho \)^2 } + \sum_{ t = \left\lceil \frac{\log T }{ \min_v \alpha_v^2 } \right\rceil }^T \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho )^2 \sqrt{ N_t^+ (J_t) } } \) \nonumber \\ 
% 		&\qquad + \frac{\rho^2}{ (1 - \rho)^2 } \sum_{t=1}^T \( \frac{4}{t^4} + \frac{1}{T} \) \tag{by Lemma \ref{lem:single-regret} and (\ref{eq:prob})} \\ 
% 		&\le \wt{ \mathcal{O} } \( \sum_{t=1}^T \frac{ poly\text{-}log (t) }{ ( 1 - \rho )^2 \sqrt{ N_t^+ (J_t)  } } \) \nonumber , \\
% 		&\le \wt{ \mathcal{O} } \( \sum_{t=1}^T \frac{ poly\text{-}log (t) }{ ( 1 - \rho )^2 \sqrt{ N_t (J_t) + \alpha_{J_t} (t - N_t (J_t ) ) - \sqrt{t \log (mT)} } } \) \tag{under event $\mathcal{E}$} , \\
% 		&\le \wt{ \mathcal{O} } \( \sum_{t=1}^T \frac{ poly\text{-}log (t) }{ ( 1 - \rho )^2 \sqrt{  \alpha_{J_t} t  - \sqrt{t \log (mT)} } } \) \nonumber  \\
% 		&\le \wt{ \mathcal{O} } \( \frac{ 1 }{ ( 1 - \rho )^2 } \sqrt{ \frac{T}{ \alpha } } \) \nonumber , 
% 	\end{align}  
% 	where $\alpha := \min_{v \in V} \alpha_v $.
	
% \textbf{Part II: $\Reg (T) = \widetilde{\mathcal{O}} \(  \frac{ 1 }{ (1 - \rho)^2 }   \sqrt{  m T } \) $. } 

% We know $ {N}_t^+ (v) \ge N_t (v) $ for all $t \in \mathbb{N}$ and $v \in V$. 
% From Lemma \ref{lem:single-regret}, we have 
% \begin{align}
%     Reg(T) \le \sum_{t=1}^T \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho)^2 \sqrt{ N_t^+ (J_t) } } \)  \le \sum_{t=1}^T \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho)^2 \sqrt{ N_t (J_t) } } \). \label{eq:tn-to-n}
% \end{align}
% Let $ t_{i,v} $ be the $i$-th time the node $v$ is played. Let $B_v$ be the total number of time node $v$ is played. Then we can regroup the sum in (\ref{eq:tn-to-n}) by 
% \begin{align*}
%     \sum_{t=1}^T \frac{1}{N_t (J_t) } = \sum_{v \in V } \sum_{i = 1}^{B_v} \frac{1}{N_{t_{ i, v }} (v ) } . 
% \end{align*}



% Since $t_{i,v}$ is the $i$-th time $v$ is played, we have $ n_{t_{ i, v } } (v) = i $. Thus we have 
% \begin{align}
%     \sum_{t=1}^T \frac{1}{N_t (J_t) } = \sum_{v \in V } \sum_{i = 1}^{B_v} \frac{1}{N_{t_{ i, v }} (v ) } =\sum_{v \in V } \sum_{i = 1}^{B_v} \frac{1}{i} \le \sum_{v \in V }  (1 + \log B_v ) \le m + m \log \frac{T}{m}, \label{eq:bound-sum-1/n}
% \end{align}
% where the last inequality uses $ \sum {B_v} = T $ and the AM-GM inequality. 

% We then insert the above results into (\ref{eq:tn-to-n}) to get 
% \begin{align}
%     \Reg(T) \le& \sum_{t=1}^T \mathcal{O} \( \frac{ poly\text{-}log (t) }{ (1 - \rho)^2 \sqrt{ N_t^+ (J_t) } } \) \nonumber \\
%     \le& \wt{\mathcal{O}}
%     \( \frac{ 1 }{ (1 - \rho)^2 }\sqrt{ T \sum_{t=1}^T \frac{1}{N_t (J_t) } } \) \tag{use the Cauchy-Schwarz inequality} \\ 
%     \le&  
%     \wt{ \mathcal{O} } \( \frac{ 1 }{ (1 - \rho)^2 } 
%      \sqrt{ T m \( 1 + \log \frac{T}{m} \) } \) \tag{use (\ref{eq:bound-sum-1/n})} \\
%     \le& \wt{ \mathcal{O} } \( \frac{ 1 }{ (1 - \rho)^2 } 
%      \sqrt{ m T } \) \nonumber, 
% \end{align}
% which concludes this part. 
% \end{proof} 

% \subsection{Proof of Theorem \ref{thm:opt}}
% \label{app:gap}

% \begin{theoremn}[\ref{thm:opt}]
% On a problem instance that satisfies Assumption \ref{assumption:transition}, Algorithm \ref{alg:opt} achieves constant regret of order $\widetilde{\mathcal{O}} \( \sum_{v: \Delta_v > 0} \( \Delta_v + \frac{1}{  (1 - \rho)^2 \Delta_v }  \) \) $, where $\widetilde{\mathcal{O}} $ omits absolute constants and logarithmic dependence on problem intrinsics. 
% \end{theoremn} 

% \begin{proof}

% % \subsubsection*{Part I: Proof for Option I.}
% % 	For a node $v$, 
%     First we define 
%     \begin{align}
% 		T_{\min, v}^{(\mathrm{2})} := \min \left\{ t \in \mathbb{N} :  t \alpha_{v}  - \sqrt{ t \log t } \ge \frac{32 \xi_t \log t }{ \Delta_v^2 } \right\} .  \label{eq:def-Tv-alg2-I} 
% 	\end{align} 
    
    
%     The proof of this theorem is developed in three steps. 
    
%     \textbf{Step 1: When $t \ge T_{\min, v}^{(2)}$, $\wt{C}_{ {N}_t^+ (v) , t } \le 2 \Delta_v$ with high probability. }
    
% 	For any $t \in \mathbb{N}$ and node $v \in V$, consider the following event. 
% 	\begin{align} 
% 		\mathcal{E}_{v,t} := \left\{ {N}_t^+ (v) - N_t(v) - (t - N_t(v))  \alpha_{v} \ge - \sqrt{ t \log t } \right\}. \label{eq:event} 
% 	\end{align} 
% % 	Since 
% 	By Lemma \ref{lem:event}, we have for any $v \in V $, with probability at least $ 1 - \frac{1}{ t^2 }$, 
% 	\begin{align} 
% 		{N}_t^+ (v) - N_t(v) - ( t - N_t (v) ) \alpha_{v} \ge - \sqrt{ t \log t } . \nonumber
% 	\end{align}  
% % 	Then by a union bound, we know $\mathcal{E}_T$ is true with probability at least $1 - \frac{1}{T}$. 
	
% 	For a sub-optimal node $v$, when 
% 	\begin{align}
% 		 {N}_t^+ (v) &\ge \frac{32 \xi_t \log t}{\Delta_v^2 },  \label{eq:req-for-t-wt} 
% 	\end{align} 
%     we have 
% 	\begin{align} 
% 		\wt{C}_{ {N}_t^+ ( v) , t} &= \wtC{ {N}_t^+ ( v ) } 
%         \le \frac{1}{2} \Delta_v . \label{eq:after-Tmin-1} 
% 	\end{align} 
	
% 	For $t \ge T_{\min, v}^{\mathrm{(2)}}$ where $T_{\min, v}^{\mathrm{(2)}}$ is defined in (\ref{eq:def-Tv-alg2-I}), under event $ \mathcal{E}_{v,t} $, we have 
% 	\begin{align}
% 	    {N}_t^+ (v) &\ge \alpha_v t  +  (1 - \alpha_v) N_t (v)  -  \sqrt{t \log t}  \tag{under event $\mathcal{E}_{v,t}$} \\
% 	    &\ge \alpha_v t  -  \sqrt{t \log t}  \tag{since $\alpha_v \le 1$} \\
% 	    &\ge \frac{ 32 \xi_t \log t }{ \Delta_v^2  }. 
% 	    \label{eq:res-step-1} 
% 	\end{align}
	
% 	From above, we know (\ref{eq:req-for-t-wt}) is true as long as $\mathcal{E}_{v,t}$ is true. Thus for any $t \ge T_{\min, v}^{\mathrm{(2)}}$, 
% 	\begin{align} 
% 	    \Pr \( \wt{C}_{ {N}_t^+ (v), t } \le \frac{1}{2} \Delta_v \) = \Pr \(  {N}_t^+ (v) \ge  \frac{ 32 \xi_t \log t }{ \Delta_v^2  } \) \ge \Pr \( \mathcal{E}_{v,t} \) \ge 1 - \frac{1}{t^2} . \nonumber
% 	\end{align} 
% 	In words, 
% 	$\wt{C}_{ {N}_t^+ (v) , t } \le \frac{1}{2} \Delta_v $ as long as (1) $t \ge T_{\min, v}^{\mathrm{(2)}}$ and (2) $\mathcal{E}_{v,t}$ is true. \\
	
% 	\textbf{Step 2: After time $T_{\min, v}^{\mathrm{(2)}}$, a sub-optimal node is played constant number of times (in expectation). } 
	
% 	For easier reference, for any $t \in \mathbb{N}$ and any $v \in V$, we write 
% 	\begin{align}
% 	    w_{v,t} := \frac{ 32 \xi_t \log t }{ \Delta_v^2  }. \label{eq:def-w} 
% 	\end{align}
	
% 	In Step 1 (Eq. \ref{eq:res-step-1}), we have shown that for any $t \ge $, event $\mathcal{E}_{v,t}$ implies  
% 	\begin{align}
% 	    {N}_t^+ (v ) \ge w_{v,t}. \label{eq:step1-summary}
% 	\end{align} 
	
% 	After time $T_{\min, v}^{\mathrm{(2)}}$, we can bound the number of times a sub-optimal arm is played (in expectation) by 
% 	\begin{align} 
%     	&\E \[ \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}} }^T \I_{ \[ J_t = v \] } \] \nonumber \\
%     	=&  \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}} }^T \left\{ \E \[ \I_{ \[ J_t = v \] } \bigg\rvert \mathcal{E}_{v,t} \] \Pr \( \mathcal{E}_{v,t} \) + \E \[  \I_{ \[ J_t = v \] } \bigg\rvert \overline{ \mathcal{E}_{v,t} } \] \( 1 - \Pr \( \mathcal{E}_{v,t} \) \) \right\} \nonumber \\ 
% 		\le& \( \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}}  }^T  \Pr \( J_t = v, t \ge {T}_{\min, v}^{\mathrm{(2)}}  \bigg\rvert \mathcal{E}_{v,t} \) \) + \sum_{t=1}^\infty \frac{1}{t^2} \nonumber \\
% 		\le& \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}}  }^T  \Pr \( J_t = v, t \ge {T}_{\min, v}^{\mathrm{(2)}}  \bigg\rvert \mathcal{E}_{v,t} \)  + \frac{\pi^2}{6} \nonumber \\
% 		\le& \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}}  }^T \Pr \( \wt{Z}_{ v, {N}_t^+  (v) } + \wt{C}_{ {N}_t^+ (v) , t } \ge \wt{Z}_{ v^*, {N}_t^+ (v^*)  } + \wt{C}_{ {N}_t^+ (v^*) , t } , \; t \ge {T}_{\min, v}^{\mathrm{(2)}} \Big\rvert \mathcal{E}_{v,t} \) + \frac{\pi^2}{6} \label{eq:use-relex-play-v-1} 
% 	\end{align} 
% 	where (\ref{eq:use-relex-play-v-1}) uses 
% 	\begin{align}
% 	    \bigg\{ \text{ a node $v$ is played at $t$ } \bigg\} \Rightarrow \bigg\{ \wt{Z}_{ v, {N}_t^+  (v) } + \wt{C}_{ {N}_t^+ (v) , t} \ge \wt{Z}_{ v^*, {N}_t^+ (v^*)  } + \wt{C}_{ {N}_t^+ (v^*) , t } \bigg\}. \nonumber
% 	\end{align}
	
% 	We then follow the argument by \cite{auer2002finite}, and bound (\ref{eq:use-relex-play-v-1}) by allowing $ {N}_t^+ (v) $ to take any values in $[w_{v,t}, t]$ (due to Eq. \ref{eq:step1-summary}), and allowing ${N}_t^+ (v^*)$ to take any values in $ [1,t] $. 
	
% 	This gives, 
% 	\begin{align}
% 	    & \Pr \( \wt{Z}_{ v, {N}_t^+ (v) } + \wt{C}_{ {N}_t^+ (v) , t } \ge \wt{Z}_{ v^*, {N}_t^+ (v^*) } + \wt{C}_{ {N}_t^+ (v^*) , t } , \; t \ge {T}_{\min, v}^{\mathrm{(2)}} \Big\rvert \mathcal{E}_{v,t} \) \nonumber \\
% 	    \le& \sum_{s = w_{v,t}}^{t} \sum_{s^* = 1}^{t} \Pr \( \wt{Z}_{ v, s } + \wt{C}_{ s , t } \ge \wt{Z}_{ v^*, s^*  } + \wt{C}_{ s^*, t }  , \; t \ge {T}_{\min, v}^{\mathrm{(2)}} \Big\rvert  \mathcal{E}_{v,t} \). \label{eq:before-three-event-1} 
% 	\end{align}
	
% % 	Since the graph structure is time-invariant, we define random variables $Z_v$ such that $ Z_v $ has the same distribution as $ \L \( \P_{t,v} \) $ for all $t$. Then, in the stochastic setting, $\Delta_v = \E \[ Z_{t,v^*}  \] -  \E \[  Z_{t,v} \] $, where $ v^* \in \arg\max_{v} \E \[ Z_{t,v} \]$. 
	
% 	As is used by \cite{auer2002finite}, when the event 
%     \begin{align}
% 	    \left\{ \wt{Z}_{ v, s } + \wt{C}_{ s, t } \ge \wt{Z}_{v^*, s^*} + \wt{C}_{ s^*, t } \right\} \nonumber 
%     \end{align} 
%     is true, at least one of the following three must be true: 
%     \begin{align}
% 	    &\wt{Z}_{ v, s } - \wt{C}_{ s, t } \le \E \[ Z_v \] , \label{eq:have-one-true1-1}
%     \\
% 	    &\wt{Z}_{ v^*, s^*  } + \wt{C}_{ s^*, t } \ge \E \[ Z_{v^*} \] , \label{eq:have-one-true2-1}
%     \\
% 	    &\E \[ Z_{v^*} \] < \E \[ Z_v \] + 2 \wt{C}_{ s, t }. \label{eq:have-one-true3-1} 
%     \end{align} 
	
% 	By Step 1 (Eq. \ref{eq:after-Tmin-1}), we know (\ref{eq:have-one-true3-1}) is false for $s \ge w_{v,t}$ and $t \ge {T}_{\min, v}^{\mathrm{(2)}} $. Thus one of (\ref{eq:have-one-true1-1}) and (\ref{eq:have-one-true2-1}) must be true. Therefore we can continue from (\ref{eq:before-three-event-1}) to get
% 	\begin{align}
% 	    &\sum_{s = w_{v,t}}^{t} \sum_{s^* = 1}^{t} \Pr \( \wt{Z}_{ v, s } + \wt{C}_{ s, t } \ge \wt{Z}_{ v^*, s^*  } + \wt{C}_{ s^*, t } , t \ge {T}_{\min, v}^{\mathrm{(2)}} \Big\rvert  \mathcal{E}_{v,t} \) \nonumber \\
% 	    \le& \sum_{s = w_{v,t}}^{t} \sum_{s^* = 1}^{t} \[ \Pr \( \wt{Z}_{ v, s } + \wt{C}_{ s, t } \le \E \[ Z_v \] \) + \Pr \( \wt{Z}_{ v, s } + \wt{C}_{ s, t } \le \E \[ Z_v \] \) \] \nonumber \\
% 	    \le& \sum_{s = w_{v,t}}^{t} \sum_{s^* = 1}^{t} \( \frac{3}{t^4} + \frac{3}{t^4} \) \label{eq:use-lem-con-1} \\
% 	    \le& \frac{6}{t^2} \label{eq:sum-prob-1}
% 	\end{align} 
% 	where (\ref{eq:use-lem-con-1}) uses Lemma \ref{lem:concentration-no-truncation}. 
	
% 	Combining (\ref{eq:use-relex-play-v-1}) and (\ref{eq:sum-prob-1}) gives 
%     \begin{align}	
%         \E \[ \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}} }^T \I_{ \[ J_t = v \] } \] \le \sum_{ t = {T}_{\min, v}^{\mathrm{(2)}} }^T \frac{6}{t^2} + \frac{\pi^2}{6} \le \frac{7 \pi^2 }{6},  
%     \end{align}
    
%     which concludes Step 2. \\
    
%     \textbf{Step 3: Up to time ${T}_{\min, v}^{\mathrm{(2)}}$, a sub-optimal node $v$ is played $\mathcal{O}\(  polylog\( {T}_{\min, v}^{\mathrm{(2)}}, \frac{1}{\Delta_v} \) \)$ number of times}
	
% % 	Applying the above result to (\ref{eq:req-for-t}), we get $\wt{C}_{ {N}_t^+ (v) , t } \le 2 \Delta_v $ when (1) $t \ge T_v$ and (2) event $\mathcal{E}_{v,t}$ is true. 
	
% 	Recall $N_t (v) $ is the number of times we play node $v$ up to time $t$. 
	
% 	For any integer $w$, we have 
% 	\begin{align}
% 		\E \[ N_{T} (v) \] &=  \E \[ \sum_{t=1}^{T} \I_{ \[ J_t = v \]  } \] \nonumber \\
% 		&\le w + \E \[ \sum_{t=1}^{t = {T}_{\min, v}^{\mathrm{(2)}}} \I_{ \[ J_t = v, \; N_{t} (v) \ge w \]  } + \sum_{t=t = {T}_{\min, v}^{\mathrm{(2)}}}^{T} \I_{ \[ J_t = v  \]  } \] \nonumber \\ 
% 		&\le w + \E \[ \sum_{t=1}^{t = {T}_{\min, v}^{\mathrm{(2)}}}  \I_{ \[ J_t = v, \; N_{t} (v) \ge w \] } \] + \frac{7\pi^2}{6} \label{eq:use-step-2-1} \\ 
% 		&\le w + \sum_{t=1}^{t = {T}_{\min, v}^{\mathrm{(2)}}} \sum_{s^* = 1}^t \sum_{s = w}^t \Pr \( \wt{Z}_{ v, s } + \wt{C}_{ s, t } \ge \wt{Z}_{ v^*, s^* } + \wt{C}_{ s^* , t } \) + \frac{7\pi^2}{6}, \label{eq:analog-step-2-1} 
% 	\end{align} 
% 	where (\ref{eq:use-step-2-1}) uses the result of Step 2, and (\ref{eq:analog-step-2-1}) uses similar argument in Step 2 (Eq. \ref{eq:use-relex-play-v-1} - \ref{eq:before-three-event-1}). 
	
% 	We set $w := \left\lceil \frac{ 32 \xi_{{T}_{\min, v}^{\mathrm{(2)}}} \log {T}_{\min, v}^{\mathrm{(2)}} }{ \Delta_v^2 } \right\rceil$, so that at time $t \le {T}_{\min, v}^{\mathrm{(2)}}$, for $s \ge w$, 
% 	\begin{align*}
% 	    \wt{C}_{s,t} = \wtC{s} \le \frac{1}{2} \Delta_v,
% 	\end{align*}
% 	which mean (\ref{eq:have-one-true3-1}) is false. 
	
% 	Also, by Lemma \ref{lem:concentration-no-truncation}, we have 
% 	\begin{align}
% 	    \Pr \[ \wt{Z}_{v, s_v} - \wt{C}_{ s_v, t } \le \E \[ Z_v \] \] \le \frac{3}{t^4}  \qquad  \Pr \[ \wt{Z}_{v^*, s^*} + \wt{C}_{ s^*, t} \ge \E \[ Z_{v^*} \]  \] \le \frac{3}{t^4} . \label{eq:quick-con-2.I}
% 	\end{align}
	
	
% 	Again we continue from (\ref{eq:analog-step-2-1}) and use  (\ref{eq:have-one-true1-1}), (\ref{eq:have-one-true2-1}) and (\ref{eq:have-one-true3-1}) to get
% 	\begin{align} 
% 		&\E \[ N_{T} (v) \] \nonumber \\
% 		\le&  
% 		\left\lceil \frac{ 32 \xi_{{T}_{\min, v}^{\mathrm{(2)}}} \log {T}_{\min, v}^{\mathrm{(2)}} }{ \Delta_v^2 } \right\rceil \nonumber \\
% 		&+ \sum_{t=1}^{T} \sum_{s^* = 1}^t \sum_{s_v = w}^t 
% 		\( \Pr \[ \wt{Z}_{v, s_v} - \wt{C}_{ s_v, t } \le \E \[ Z_v \] \]   + \Pr \[ \wt{Z}_{v^*, s^*} + \wt{C}_{ s^*, t} \ge \E \[ Z_{v^*} \]  \]  \) + \frac{7 \pi^2 }{6} \\
% 		\le& \frac{ 32 \xi_{{T}_{\min, v}^{\mathrm{(2)}}} \log {T}_{\min, v}^{\mathrm{(2)}} }{ \Delta_v^2 } + 1 + \frac{13 \pi^2}{6} ,
% 	\end{align} 
% 	where on the last line we use (\ref{eq:quick-con-2.I}). 
	
% 	Finally, since $\Reg (T) = \sum_{v \in [K]} \Delta_v \E \[ N_T(v) \]$, we have 
% 	\begin{align}
% 	    Reg(T) \le \sum_{v: \Delta_v > 0} \[  \frac{ 32 \xi_{{T}_{\min, v}^{\mathrm{(2)}}} \log {T}_{\min, v}^{\mathrm{(2)}} }{ \Delta_v } + \( 1 + \frac{13 \pi^2}{6} \) \Delta_v \] , \nonumber
% 	\end{align} 
% 	where $ 
% 	{T}_{\min, v}^{\mathrm{(2)}} = 
% 	\widetilde{\mathcal{O}} \( \frac{ 1 }{ \alpha_v (1 - \rho)^2 \Delta_v^2 } \) 
% 	$ 
% 	and $ 
% 	\xi_{{T}_{\min, v}^{\mathrm{(2)}}} = 
% 	\widetilde{ \mathcal{O} } \( \frac{1}{ \( 1 - \rho \)^2 } \)
% 	$. 
% \end{proof}
